A sufficient set of experimentally implementable thermal operations

Recent work using tools from quantum information theory has shown that at the nanoscale where quantum effects become prevalent, there is not one thermodynamical second law but many. Derivations of these laws assume that an experimenter has very precise control of the system and heat bath. Here we show that these multitude of laws can be saturated using two very simple operations: changing the energy levels of the system and thermalizing over any two system energy levels. Using these two operations, one can distill the optimal amount of work from a system, as well as perform the reverse formation process. Even more surprisingly, using only these two operations and one ancilla qubit in a thermal state, one can transform any state into any other state allowable by the second laws. We thus have the remarkable result that the second laws hold for fine-grained manipulation of system and bath, but can be achieved using very coarse control. This brings the full array of thermal operations into a regime accessible by experiment, and establishes the physical relevance of these second laws.

==> Supplementary_Material/Supplementary_cp.tex <==
\appendix
\section{Preliminaries}


In this appendix, we recall and define relevant concepts and results from the resource theory of thermal operations (TO).



\subsection{Thermal Operations} \label{ssec:thermal operations}

The resource theory of thermal operations \cite{janzing2000thermodynamic, horodecki2013fundamental} models the thermodynamics of a small system in the presence of a large heat bath. Given a system in state $\rho$ with Hamiltonian $H$ and such a heat bath at temperature $T$, the following operations can be applied:
\begin{enumerate}
\item An ancillary system with any Hamiltonian, in the Gibbs state of that Hamiltonian at temperature $T$, can be appended as an ancilla. For the Hamiltonian $H_B=\sum_{i=1}^{n} E_i \ketbra{i}{i}$, the corresponding Gibbs state at temperature $T$ is defined as:
\begin{equation}
\tau_B=\frac{1}{Z_B}\sum_{i=1}^{n}e^{-\beta E_i} \ketbra{i}{i},
\end{equation}
where $\beta$ is the inverse temperature and $Z_B=\sum_{i=1}^{n} e^{-\beta E_i}$ is the partition function.
\item Any energy-conserving unitary, i.e. those unitaries that commute with the total Hamiltonian, can be applied to the global system.
\item Any subsystem can be discarded through tracing out.
\end{enumerate}
Given these, the action of a thermal operation on the state $\rho$ of a state-Hamiltonian pair $\left(\rho,H_S\right)$ at temperature $T$ can be written: 
\begin{equation}
\rho\stackrel{\textrm{TO}}{\longrightarrow}\tr_A\left[U\left(\rho\otimes\tau_B\right)U^\dagger\right],
\end{equation}
where $\tau_B$ is the Gibbs state of a Hamiltonian $H_B$, $A$ is the subsystem to be discarded and $U$ is a unitary such that:
\begin{equation}
\left[U,H_S+H_B\right]=0,
\end{equation}
and we have used the shorthand notation $H_S+H_B=H_S\otimes\id_B+\id_S\otimes H_B$.

\subsection{Thermo-majorization} \label{ss:thermomaj}

Suppose we have a system $\left(\rho,H_S\right)$. Determining whether it can be transformed into the system $\left(\sigma,H_S\right)$ using thermal operations, can be formulated using thermo-majorization diagrams \cite{horodecki2013fundamental}. 
\begin{definition}[Thermo-majorization diagrams]
Given an $n$-level system, let $H_S=\sum_{i=1}^{n}E_i \ketbra{i}{i}$ be the system's Hamiltonian and the state of the system be block-diagonal in the energy eigenbasis and given by $\rho=\sum_{i=1}^{n}\eta_i \ketbra{i}{i}$. To define the thermo-majorization curve of $\rho$, we first $\beta$-order the eigenvalues and energy levels, listing them such that $\eta_i e^{\beta E_i}$ is in non-increasing order. 

The thermo-majorization curve of $\rho$ is then formed by plotting the $\beta$-ordered points:
\begin{equation} \label{eq:th-maj set}
\left\{\sum_{i=1}^{k} e^{-\beta E^{\left(\rho\right)}_i},\sum_{i=1}^{k} \eta_i^{\left(\rho\right)}\right\}_{k=1}^{n},
\end{equation}
together with $\left(0,0\right)$, and connecting them piecewise linearly to form a concave curve. Here, the superscript $\left(\rho\right)$ on $E_i$ and $\eta_i$ indicate that they have been $\beta$-ordered and that this ordering depends on $\rho$.
\end{definition}

An example of thermo-majorization diagrams is shown in Figure \ref{fig:thermo diagrams}. We say that one block-diagonal state, thermo-majorizes another if its thermo-majorization curve never lies below that of the other. If $\rho$ is not block-diagonal in the energy eigenbasis, determining whether a transition is possible or not can be written in terms of the state formed by decohering $\rho$ in the energy eigenbasis. This state $\mathcal{D}\left(\rho\right)$ is given by:
\begin{equation}
\mathcal{D}\left(\rho\right)=\sum_{i=1}^{n}\ketbra{i}{i}\rho\ketbra{i}{i},
\end{equation}
where $\left\{\ket{i}\right\}_{i=1}^{n}$ are the eigenvectors of the systems Hamiltonian. The operation of decohering $\rho$ to create $\mathcal{D}\left(\rho\right)$ can be performed using a thermal operation that commutes with all other thermal operations \cite{brandao2013resource}.
\begin{figure}
\centering
\includegraphics[width=0.7\columnwidth]{supplementary_figures/Thermo-majorizationgraph.pdf}
\caption[Thermo-majorization curves.]{\emph{Thermo-majorization curves.} \emph{a)} The thermo-majorization curve for a block-diagonal state, $\rho$, is defined by plotting the points: $\left\{\sum_{i=1}^{k} e^{-\beta E_i^{\left(\rho\right)}},\sum_{i=1}^{k}\eta_i^{\left(\rho\right)}\right\}_{k=1}^{n}$. Note that states associated with the same Hamiltonian may have different $\beta$-orderings, as illustrated by $\rho$ and $\sigma$ here. \emph{b)} Here, $\rho$ thermo-majorizes $\sigma$ as the thermo-majorization curve of $\rho$ is never below the thermo-majorization curve of $\sigma$. \emph{c)} The thermo-majorization curve of a Gibbs state is given by a straight line between $\left(0,0\right)$ and $\left(Z,1\right)$. All other states thermo-majorize it. \emph{d)} The pure state corresponding to the highest energy level of an $n$-level system thermo-majorizes all other states associated with that Hamiltonian. \emph{e)} We call a point on a curve an elbow, if the gradient of the curve changes as it passes through the point. Otherwise, it is a non-elbow.}
\label{fig:thermo diagrams}
\end{figure}



With these definitions in place, we can give the result of \cite{horodecki2013fundamental}:
\begin{theorem}[Thermo-majorization] Given two states $\rho$ and $\sigma$ of an $n$-level system with Hamiltonian $H_S$:
\begin{enumerate}
\item If $\rho$ and $\sigma$ are block-diagonal in the energy eigenbasis, then $\rho\stackrel{\textrm{TO}}{\longrightarrow}\sigma$, if and only if $\rho$ thermo-majorizes $\sigma$.
\item If $\sigma$ is block-diagonal in the energy eigenbasis, then $\rho\stackrel{\textrm{TO}}{\longrightarrow}\sigma$, if and only if $\mathcal{D}\left(\rho\right)$ thermo-majorizes $\sigma$.
\item In general, $\rho\stackrel{\textrm{TO}}{\longrightarrow}\sigma$, only if $\mathcal{D}\left(\rho\right)$ thermo-majorizes $\mathcal{D}\left(\sigma\right)$.
\end{enumerate}
\end{theorem}

\subsection{Wits and switch qubits} \label{ssec:wits&switch}

\subsubsection{Work} \label{ssec:wits}

In general, if we want a transition from $\rho$ to $\sigma$ to be possible, work may have to be added. Alternatively, if a transition can be achieved with certainty, it can be possible to extract work. Within the thermal operations framework, the optimal amount of work that must be added or can be gained, the work of transition, can be quantified using a continuous system, or for example the energy gap $W$ of a 2-level system, a wit \cite{horodecki2013fundamental}, with zero energy state $\ket{0}$ and an additional state $\ket{1}$. The associated Hamiltonian is:
\begin{equation}
H_W= W\ketbra{1}{1}.
\end{equation}
The work of transition, denoted $\Wtran{\rho}{\sigma}$, is then defined to be the greatest value of $W$ such that the following holds:
\begin{equation}\label{eq:work def}
\left(\rho\otimes\ketbra{0}{0},H_S+H_W\right)\stackrel{\textrm{TO}}{\longrightarrow}\left(\sigma\otimes\ketbra{1}{1},H_S+H_W\right).
\end{equation}
If $\Wtran{\rho}{\sigma}$ is negative, to convert $\rho$ into $\sigma$ work has been taken from the work storage system to enable the transition to take place. On the other hand, if $\Wtran{\rho}{\sigma}$ is positive, in converting $\rho$ into $\sigma$ it has been possible to store some extracted work in the work system.

Defining work in such a way enables the quantification of the worst-case work of a process.  When $\Wtran{\rho}{\sigma}$ is negative, it can be interpreted as the smallest amount of work that must be supplied to guarantee the transition. If it is positive, it is the largest amount of work we are guaranteed to extract in the process. As the work system is both initially and finally in a pure state, no entropy is stored in it and its energy change must be completely due to work being exchanged with the system.  One can also quantify average work.

\subsubsection{Changes of Hamiltonian}

Thermodynamics is not just concerned with a system with Hamiltonian $H$ and whether it is possible to transform $\rho$ into $\sigma$ whilst keeping the $H$ fixed. One also wants to be able to consider transitions where the Hamiltonian changes, i.e.:
\begin{equation}
\left(\rho,H_1\right)\longrightarrow\left(\sigma,H_2\right),
\end{equation}
and to determine the work cost or yield of performing such a change. Following \cite{horodecki2013fundamental}, this scenario can be mapped to one with identical initial and final Hamiltonian using the \emph{switch qubit} construction. Here, we instead consider the transition between $\left(\rho\otimes\ketbra{0}{0}\right)$ and $\left(\sigma\otimes\ketbra{1}{1}\right)$ with Hamiltonian:
\begin{equation} \label{eq:Ham change}
H=H_1\otimes\ketbra{0}{0}+H_2\otimes\ketbra{1}{1}.
\end{equation}
Note that the partition function associated with $H$ is $Z=Z_1+Z_2$, where $Z_1$ and $Z_2$ are the partition functions of $H_1$ and $H_2$ respectively.

To model the work of transition in such a process, we combine this with Eq. \eqref{eq:work def} to give:
\begin{equation}
\left(\rho\otimes\ketbra{0}{0}\otimes\ketbra{0}{0},H+H_{W}\right)\stackrel{\textrm{TO}}{\longrightarrow}\left(\sigma\otimes\ketbra{1}{1}\otimes\ketbra{1}{1},H+H_{W}\right),
\end{equation}
and maximize over $W$.




\newpage

\section{\longCOs\ as thermal operations} \label{sec:coarseops}

In this appendix, we show how the \longCO\ (\CO) we have introduced can be realized using thermal operations. 

Under \longCOs\ the following operations can be applied:
\begin{enumerate}
\item A single 2-level system with known Hamiltonian, in the Gibbs state of that Hamiltonian at temperature $T$, can be appended as an ancilla.
\item \longPLT\ (\PLT) over any subset of energy levels.
\item \longLTs\ (\LT), provided the work cost is accounted for.
\item The ancilla system may be discarded.
\item Any energy conserving unitary $U$ such that $\left[U,H_S\right]$ may be applied to the system. \chris{I've added this so our results apply to block-diagonal states and not just diagonal ones. Also, with this we can now decohere in the energy eigenbasis so we can reproduce all transformations where the target state is block-diagonal.}
\end{enumerate}
Operation 1 can obviously be realized using Operation 1 of thermal operations as described in Appendix \ref{ssec:thermal operations} but as we restrict to one ancillary system, the converse does not hold. As we shall see, Operation 2 can be realized using thermal operations whilst in general, Operation 3 may cost work to perform. Operation 5 allows us to decohere in the energy eigenbasis (by applying a random energy conserving unitary) and to treat all block-diagonal states as being diagonal in the energy eigenbasis. As the unitary is applied only to the system under consideration, it is much easier to implement experimentally than the more general Operation 2 of thermal operations.

\subsection{\longPLTs}

\longPLTs\ act on a subset of a system's energy levels, partially thermalizing the state supported on those levels. More formally:
\begin{definition}[\longPLT]
Given an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$, a \longPLT\ is parametrized by $\lambda\in\left[0,1\right]$ and acts on some subset of the system's energy levels. Denote this subset of energy levels by $\mathcal{P}$ and the \longPLT\ by $\PLT_{\mathcal{P}}\left(\lambda\right)$.

The action of $\textrm{\PLT}_{\mathcal{P}}\left(\lambda\right)$ on $\rho=\sum_{i=1}^{n}\eta_i\ketbra{i}{i}$, is defined by:
\begin{equation}
\rho\stackrel{\textrm{\PLT}_{\mathcal{P}}\left(\lambda\right)}{\longrightarrow} \rho',
\end{equation}
where $\rho'=\sum_{i=1}^{n} \eta'_i\ketbra{i}{i}$ and the $\eta'_i$ are such that for $i\in\mathcal{P}$:
\begin{equation} \label{eq:PLT components}
\eta'_i=\left(1-\lambda\right)\eta_i + \frac{\lambda e^{-\beta E_i}}{\sum_{i\in\mathcal{P}}e^{-\beta E_i}}\sum_{i\in\mathcal{P}}\eta_i,
\end{equation}
and $\eta'_i=\eta_i$ otherwise. The action of a \longPLT, is illustrated in terms of thermo-majorization curves in Figure \ref{fig:PT}.
\end{definition}
\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{article_figures/PLTGraph.pdf}
\caption{\emph{Action of \longPLT.} Here we illustrate the action of \PLTs\ applied to a state $\rho$ over the two energy levels between points $A$ and $B$ for various degrees of thermalization. Note, that as we apply the \PLTs\ to adjacent energy levels with respect to the $\beta$-ordering of $\rho$, the final states maintain this $\beta$-order.} 
\label{fig:PT}
\end{figure}

% Original figure
%\begin{figure}
%\centering
%\begin{subfigure}{.5\textwidth}
%  \centering
%  \includegraphics[width=.9\linewidth]{figures/pt_1.pdf}
%  \caption{Initial state.}
%  \label{fig:PT initial}
%\end{subfigure}%
%\begin{subfigure}{.5\textwidth}
%  \centering
%  \includegraphics[width=.9\linewidth]{figures/pt_2.pdf}
%  \caption{Final state.}
%  \label{fig:PT final}
%\end{subfigure}
%\caption{\emph{Action of \longPLT.} Here the initial state is fully thermalized ($\lambda=1$) over the three energy levels between points 1 and 2 on the thermo-majorization diagram. This results in the final state. \chris{Do we want to show an example with $\lambda<1$? Perhaps superimpose it on the second diagram, or combine all three curves on one diagram.}}
%\label{fig:PT}
%\end{figure}


Note that such an operation preserves the $\beta$-ordering of the levels in $\mathcal{P}$ as, for $i,j\in\mathcal{P}$, if $\eta_i e^{\beta E_i}\geq \eta_j e^{\beta E_j}$, then  $\eta'_i e^{\beta E_i}\geq \eta'_j e^{\beta E_j}$. In particular, if for some $d$, $\mathcal{P}=\left\{i^{\left(\rho\right)}\right\}_{i=k}^{k+d-1}$ (with the superscript $\left(\rho\right)$ denoting that the energy levels are $\beta$-ordered with respect to $\rho$), then $\rho'$ will have the same $\beta$-ordering as $\rho$. 

That \longPLT\ form a subset of thermal operations, is captured in the following Lemma.
\begin{lemma} \label{le:PLT as TO}
The map $\textrm{\PLT}_{\mathcal{P}}\left(\lambda\right)$ can be implemented using thermal operations.
\end{lemma}
\begin{proof}
To show this, we give an explicit protocol implementing a \longPLT. For simplicity, we assume $\lambda$ is a positive rational of the form $\frac{a}{b}$ (if $\lambda$ is irrational, then $a$ and $b$ should be chosen such that the \longPLT\ is implemented to the desired accuracy). Let the state of the system be $\rho=\sum_{i=1}^{n}\eta_i\ketbra{i}{i}$ and the associated Hamiltonian, $H_S=\sum_{i=1}^{n}E_i\ketbra{i}{i}$. The protocol then runs as follows:
\begin{itemize}
\item Step 1. Using Operation 1 of thermal operations:
\begin{equation*}
\left(\rho,H_S\right)\rightarrow\left(\rho\otimes\tau_A\otimes\id_b,H_S+H_A+H_M\right),
\end{equation*}
where $\tau_A$ is the Gibbs state of a $|\mathcal{P}|$-level system with Hamiltonian:
\begin{equation*}
H_A=\sum_{j\in\mathcal{P}} E_j \ketbra{j}{j},
\end{equation*}
and $\id_b$ is the maximally mixed state of dimension $b$. This is a Gibbs state of the $b$-level system with Hamiltonian $H_M=0$.
\item Step 2. Let $\left\{\ket{r_S,s_A,t_M}\right\}$ be the set of orthonormal eigenvectors of $H_S+H_A+H_M$, each with associated energy level $E_r+E_s$. The eigenvalue of $\rho\otimes\tau_A\otimes\id_b$ associated with each energy level is $\frac{1}{bZ_A}\eta_r e^{-\beta E_s}$. Let $U$ be a unitary acting on the global system such that for $r \in \mathcal{P}$, $\forall s$, $t\in\left\{1,\dots,a\right\}$:
\begin{equation*}
U\ket{r_S,s_A,t_M}=\ket{s_S,r_A,t_M},
\end{equation*}
and $U\ket{r_S,s_A,t_M}=\ket{r_S,s_A,t_M}$ otherwise. By construction, $U$ is an energy conserving unitary that commutes with the total Hamiltonian.
\item Step 3. Discard the two ancilla systems.
\end{itemize}
After applying this protocol, the population of energy level $E_j$ for $j\in\mathcal{P}$ is:
\begin{align*}
&\eta_j - \frac{a}{bZ_A}\sum_{i\in\mathcal{P}}e^{-\beta E_i}\eta_j + \frac{a}{bZ_A}\sum_{i\in\mathcal{P}}e^{-\beta E_j}\eta_i,\\
=&\left(1-\frac{a}{b}\right)\eta_j+\frac{a}{b}\frac{e^{-\beta E_j}}{\sum_{i\in\mathcal{P}}e^{-\beta E_i}}\sum_{i\in\mathcal{P}}\eta_i,
\end{align*}
and $\eta_j$ otherwise. Comparing this with Eq.~\eqref{eq:PLT components}, we see that we have implemented the \longPLT\ as required.
\end{proof}


\subsection{\longLT}

\longLTs\ adjust the energy levels of a system's Hamiltonian while keeping the state of the system fixed.
\begin{definition}[\longLT]
Given an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ in the state $\rho=\sum_{i=1}^{n}\eta_i\ketbra{i}{i}$, a \longLT\ is parametrized by a set of real numbers $\mathcal{E}=\left\{h_i\right\}_{i=1}^{n}$ and denoted by $\LT_{\mathcal{E}}$.

The action of $\LT_{\mathcal{E}}$ on $\left(\rho,H_S\right)$ is:
\begin{equation}
\left(\rho,H_S\right)\stackrel{\LT_{\mathcal{E}}}{\longrightarrow}\left(\rho,H'_S\right),
\end{equation}
where:
\begin{equation}
H'_S=\sum_{i=1}^{n}\left(E_i+h_i\right)\ketbra{i}{i}.
\end{equation}

The single-shot, worst-case, work cost/yield of $\LT_{\mathcal{E}}$ is defined by:
\begin{equation} \label{eq:LT cost}
W_{\LT_{\mathcal{E}}}=-\max_{i:\eta_i>0} h_i.
\end{equation}
If $W_{\LT_{\mathcal{E}}}$ is negative, work must be added for the transformation to happen deterministically while if it is positive, it may be possible to extract some work.
\end{definition}
The action of a \longLT, is illustrated in terms of thermo-majorization curves in Figure \ref{fig:LT}.

\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{article_figures/LTGraph.pdf}
\caption{\emph{Action of \longLTs.} Here we illustrate the action of \LTs\ applied to a system with state-Hamiltonian pair $\left(\rho,H\right)$. Note that \LTs\ leave the occupation probabilities of $\rho$ unchanged but may alter the $\beta$ ordering.} 
\label{fig:LT}
\end{figure}

\longLT\ can be modeled within thermal operations using the wit and switch qubit introduced in Appendix \ref{ssec:wits&switch}.
\begin{lemma}
The map $\LT_{\mathcal{E}}$ can be implemented using thermal operations with work cost at most $W_{\LT_{\mathcal{E}}}$.
\end{lemma}
\begin{proof}
Let $H=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ be the initial Hamiltonian and $H'=\sum_{i=1}^{n} E'_i\ketbra{i}{i}$ be the final Hamiltonian after the application of $\LT_{\mathcal{E}}$. Let $\mathcal{E}=\left\{h_i\right\}_{i=1}^{n}$ so $E'_i=E_i+h_i$.

Consider modeling this transformation using the switch qubit construction:
\begin{equation*}
H_T=H\otimes\ketbra{0}{0}+H'\otimes\ketbra{1}{1}.
\end{equation*}
Let $H_W=W\ketbra{1}{1}$ be the Hamiltonian for the wit. The work require to implement the \longLT\, and convert the system $\left(\rho,H\right)$ into $\left(\rho,H'\right)$ under thermal operations $W_{H\rightarrow H'}$ is then given by the largest value of $W$ such that:
\begin{equation*}
\left(\rho\otimes\ketbra{0}{0}\otimes\ketbra{0}{0},H_T+H_W\right)\stackrel{\textrm{TO}}{\longrightarrow}\left(\rho\otimes\ketbra{1}{1}\otimes\ketbra{1}{1},H_T+H_W\right).
\end{equation*}

To see that $W_{H\rightarrow H'} \geq W_{\LT_{\mathcal{E}}}$, consider the \longLT\ parametrized by $\tilde{\mathcal{E}}=\left\{\tilde{h}_i\right\}_{i=1}^{n}$ where $\tilde{h}_i=W_{\LT_{\mathcal{E}}}$, $\forall i$. Let $\tilde{H}$ denote the Hamiltonian obtained by applying $\LT_{\tilde{\mathcal{E}}}$ to $H$ and note that the \longLT\ is such that $W_{\LT_{\mathcal{E}}}=W_{\LT_{\tilde{\mathcal{E}}}}$. To model this \longLT\ using thermal operations let:
\begin{equation*}
\tilde{H}_T=H\otimes\ketbra{0}{0}+\tilde{H}\otimes\ketbra{1}{1},
\end{equation*}
and its work cost under thermal operations $W_{H\rightarrow \tilde{H}}$ is given by the largest value of $W$ such that:
\begin{equation*}
\left(\rho\otimes\ketbra{0}{0}\otimes\ketbra{0}{0},\tilde{H}_T+H_W\right)\stackrel{\textrm{TO}}{\longrightarrow}\left(\rho\otimes\ketbra{1}{1}\otimes\ketbra{1}{1},\tilde{H}_T+H_W\right).
\end{equation*}
It can easily be seen that $W_{H\rightarrow \tilde{H}}=W_{\LT_{\tilde{\mathcal{E}}}}$ and $W_{H\rightarrow \tilde{H}}\leq W_{H\rightarrow H'}$. Hence the result follow.
\end{proof}

Note that this result implies that implementing the effect of a \longLT\ using a switch qubit and thermal operations, can be more cost-effective (in terms of work required to make the transformation deterministically) then performing a \longLT\ itself.

\subsection{\longITRs\ and \longPFs} \label{ssec:points flow}

We can combine sequences of \longLTs\ and \longPLTs\ in such a way to form a useful protocol, termed an \emph{\longITR}\ as they are similar in construction to the Isothermal Reversible Processes considered in \cite{aaberg2013truly} but require \longPLTs\ rather than full thermalizations. In terms of thermo-majorization curves, \longITRs\ will enable us to move non-elbow points along the segments on which they exist, without changing the shape and structure of the rest of the curve. More formally:
\begin{definition}[\longITR] \label{def:ITR}
Given an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$, an \longITR\ is parametrized by a positive constant $\kappa$ and acts on some pair of the system's energy levels, indexed by $j$ and $k$. Denote the \longITR\ by $\ITR_{j,k}\left(\kappa\right)$.

The action of $\ITR_{j,k}\left(\kappa\right)$ on $\left(\rho,H_S\right)$ where $\rho=\sum_{i=1}^{n}\eta_i\ketbra{i}{i}$, is defined by:
\begin{equation}
\left(\rho,H_S\right)\stackrel{\ITR_{j,k}\left(\kappa\right)}{\longrightarrow} \left(\rho',H'_S\right),
\end{equation}
where $\rho'=\sum_{i=1}^{n}\eta'_i$ and $H'_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$. Defining $\tilde{\eta}_j=\frac{e^{-\beta E_j}}{e^{-\beta E_j}+e^{-\beta E_k}}\left(\eta_j+\eta_k\right)$ and $\tilde{\eta}_k=\frac{e^{-\beta E_k}}{e^{-\beta E_j}+e^{-\beta E_k}}\left(\eta_j+\eta_k\right)$, the components of $\left(\rho',H'_S\right)$ in terms of $\kappa$ are then:
\begin{align} 
\begin{split} \label{eq:ITR components}
\eta'_j&=\tilde{\eta}_j e^{-\beta\kappa},\\
\eta'_k&=\tilde{\eta}_k +\left(1-e^{-\beta \kappa}\right)\tilde{\eta}_j,  \\
E'_j&=E_j+\kappa,       \\
E'_k&=-\frac{1}{\beta} \ln\left[e^{-\beta E_k}+e^{-\beta E_j} \left(1-e^{-\beta \kappa}\right)\right],
\end{split}
\end{align}
with $\eta'_i=\eta_i$ and $E_i=E'_i$ for $i\notin\left\{j,k\right\}$. 
\end{definition}
The action of an \longITR\ in terms of therm-majorization diagrams is illustrated in Figure \ref{fig:ITR}.
\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{article_figures/ITRgraph.pdf}
\caption{\emph{Action of \longITRs.} Here we illustrate the action of \ITRs\ applied to a system with state-Hamiltonian pair $\left(\rho,H\right)$. Using \ITRs, the point at $C$ can be moved such that it lies anywhere on the line-segment between $A$ and $B$ and without changing the shape of the overall thermo-majorization curve. By performing this process sufficiently slowly, this can be done with no deterministic work cost. If one moves the point $C$ to coincide with point $A$ (respectively $B$), one can then use a second \ITR\ to move point $A$ ($B$) as illustrated by the dashed arrows. Again, this does not alter the shape of the thermo-majorization curve.} 
\label{fig:ITR}
\end{figure}


Note that in such a process, $Z_S=Z'_S$ and that for all $\kappa$:
\begin{equation} \label{eq:ITR relation}
\eta'_j e^{\beta E'_j}=C=\eta'_k e^{\beta E'_k},
\end{equation}
where $C$ is some constant.

The work cost of an \longITR\ is captured in the following Lemma:
\begin{lemma} \label{le:ITR cost}
The operation $\ITR_{j,k}\left(\kappa\right)$ does not cost any work.
\end{lemma}
\begin{proof}
To show this, we define a $t$-step procedure that implements $\ITR_{j,k}\left(\kappa\right)$ with each step consisting of a \longLT\ and a \longPLT. Let $\left(\rho,H_S\right)$ and $\left(\rho',H'_S\right)$ be defined as per Definition \ref{def:ITR}. Without loss of generality, assume that:
\begin{equation*}
\eta_j e^{\beta E_j}=C=\eta_k e^{\beta E_k}.
\end{equation*}
for some constant $C$ (if not, we can always perform $\textrm{\PLT}_{\left\{j,k\right\}}\left(\lambda=1\right)$ to make it so and as by Lemma \ref{le:PLT as TO} this is a thermal operation, this costs no work). Hence in the language of Definition \ref{def:ITR}, $\eta_j=\tilde{\eta}_j$ and $\eta_k=\tilde{\eta}_k$.

Define  $\epsilon=\frac{E'_j-E_j}{t}$. Let the Hamiltonian after step $r$ be $H^{\left(r\right)}_S=\sum_{i=1}^{n}E^{\left(r\right)}_i\ketbra{i}{i}$ and the state of the system be $\rho^{\left(r\right)}=\sum_{i=1}^{n}\eta^{\left(r\right)}\ketbra{i}{i}$. In step $r$, we perform the level transformation such that:
\begin{align*}
E^{\left(r\right)}_j&=E_j+r\epsilon,\\
E^{\left(r\right)}_k&=-\frac{1}{\beta}\ln\left[e^{-\beta E_k}+e^{-\beta E_j}\left(1-e^{-\beta r\epsilon}\right)\right]
\end{align*}
and fully thermalize over energy levels $j$ and $k$ so that:
\begin{align*}
\eta^{\left(r\right)}_j&=\eta_j e^{-\beta r\epsilon},\\
\eta^{\left(r\right)}_k&=\eta_k+\left(1-e^{-\beta r\epsilon}\right)\eta_j.
\end{align*}
All other energy levels and occupation probabilities remain unchanged. It can readily be verified that $Z^{\left(r\right)}_S=Z_S$ and that:
\begin{equation*}
\eta^{\left(r\right)}_j e^{\beta E^{\left(r\right)}_j}=C=\eta^{\left(r\right)}_k e^{\beta E^{\left(r\right)}_k}.
\end{equation*}
Hence, this protocol produces the desired $\left(\rho',H_{S'}\right)$ after $t$ steps. 

Such a protocol alters the state and Hamiltonian of the system but does not change the shape of the system's thermo-majorization curve. Following the proof of \cite[Supplementary Lemma 1.]{aaberg2013truly} regarding Isothermal Reversible Processes, we shall now show that the work cost of this protocol becomes increasingly peaked around zero as the number of steps taken tends to infinity.

Let $W^{\left(r\right)}$ denote the random variable for the work distribution in step $r$ of the \ITR. The work distribution for the whole $t$-step \ITR\ process is then:
\begin{equation*}
W^{\ITR}=\sum_{r=1}^{t}W^{\left(r\right)}.
\end{equation*}
Using Eqs. \eqref{eq:ITR components} and \eqref{eq:ITR relation}, $W^{\left(r\right)}$ is such that with probability:
\begin{align*}
C e^{-\beta E_j^{\left(r\right)}}, &\quad W^{\left(r\right)}=\epsilon,\\
C e^{-\beta E_k^{\left(r\right)}}, &\quad W^{\left(r\right)}=-\frac{1}{\beta}\ln\left[e^{-\beta E^{\left(r\right)}_k}+e^{-\beta E^{\left(r\right)}_j}\left(1-e^{-\beta\epsilon}\right)\right]-E^{\left(r\right)}_k,\\
\textrm{otherwise}, &\quad W^{\left(r\right)}=0.
\end{align*}
Now, for large $t$, small $\epsilon$, this becomes such that with probability:
\begin{align*}
C e^{-\beta E_j^{\left(r\right)}}, &\quad W^{\left(r\right)}=\epsilon,\\
C e^{-\beta E_k^{\left(r\right)}}, &\quad W^{\left(r\right)}=-\epsilon e^{\beta\left(E^{\left(r\right)}_k-E^{\left(r\right)}_j\right)}+O(\epsilon^2),\\
\textrm{otherwise}, &\quad W^{\left(r\right)}=0.
\end{align*}
Hence as $t\rightarrow\infty$, $\left\langle W^{\left(r\right)}\right\rangle\rightarrow0$, for all $r$. As $t=\frac{E^{(t)}_j-E^{(0)}_j}{\epsilon}=\frac{E'_j-E_j}{\epsilon}$, we have that:
\begin{equation*}
\left\langle W^{\ITR}\right\rangle=\sum_{r=1}^{t}\left\langle W^{\left(r\right)}\right\rangle\rightarrow 0, \quad \textrm{as } t\rightarrow\infty.
\end{equation*}

Now consider the variance of $W^{\ITR}$. For large $t$, hence small $\epsilon$:
\begin{align*}
\left\langle {W^{\left(r\right)}}^2\right\rangle &= C e^{-\beta E^{\left(r\right)}_j}\epsilon^2+C e^{-\beta E^{\left(r\right)}_k}\epsilon^2 e^{2\beta\left(E^{\left(r\right)}_k-E^{\left(r\right)}_j\right)}+O(\epsilon^4)\\
&=C e^{-\beta E^{\left(r\right)}_j}\epsilon^2 \left(1 + e^{\beta\left(E^{\left(r\right)}_k-E^{\left(r\right)}_j\right)}\right)+O(\epsilon^4)\\
&\rightarrow 0 \quad \textrm{as } \epsilon\rightarrow 0.
\end{align*}
Hence, $\textrm{Var}\left(W^{\left(r\right)}\right)\rightarrow 0$ as $t\rightarrow \infty$. As the $W^{\left(r\right)}$ are independent:
\begin{align*}
\textrm{Var}\left(W^{\ITR}\right)&=\sum_{r=1}^{t}\textrm{Var}\left(W^{\left(r\right)}\right)\\
&\rightarrow 0 \quad \textrm{as } \epsilon\rightarrow 0.
\end{align*}

Note that this analysis extends to the case where $E'_j\rightarrow\infty$. If we parametrize $E'_j$ in terms of the number of steps taken in the \ITR\ protocol so that $E'_j=\ln t$, then in the limit $t\rightarrow\infty$, $E'_j\rightarrow\infty$, $\left\langle W^{\ITR}\right\rangle\rightarrow 0$  and $\textrm{Var}\left(W^{\ITR}\right)\rightarrow0$.

Now, Chebyshev's inequality gives us that:
\begin{align*}
P\left(\left|W^\ITR\right|\geq k\sqrt{\textrm{Var}\left(W^{\ITR}\right)}\right)\leq \frac{1}{k^2},
\end{align*}
so by taking $t$ and $k$ to be large, we obtain that the work distribution for the \ITR\ becomes increasingly peaked around 0.
\end{proof}

Hence, \longITRs\ can be used to move non-elbow points along straight-line segments of a thermo-majorization curve, using \longCOs\ and without expending any work. By combining two \ITRs, it is possible to commute non-elbow points with elbows, meaning that non-elbows can be moved to any point of the thermo-majorization curve for free. We term this operation \emph{Exact \longPF}.
\begin{definition}[Exact \longPF\ (E\PF)] \label{def:EPF}
Exact \longPF\ is illustrated in Figure \ref{fig:exact PF}. Given an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ and state $\rho=\sum_{i=1}^{n} \eta_i\ketbra{i}{i}$ such that:
\begin{equation} \label{eq:exact PF elbow}
\eta_j e^{\beta E_j}=\eta_k e^{\beta E_k},
\end{equation}
for some $j,k$ (i.e. there is a non-elbow point on the thermo-majorization curve), an Exact \longPF\ moves this non-elbow to another part of the thermo-majorization curve whilst keeping the shape of the curve fixed.  
\end{definition}
To implement E\PF, we first apply a \ITR\ that sends $E_j\rightarrow\infty$. This lowers the energy of $E_k$ and does not alter the shape of the thermo-majorization curve. Next, to move the non-elbow to another part of the curve, we apply another \ITR\ to $j$ and a third level labeled by $l$, bringing the energy level associated with $j$ back down from infinity to some $E'_j$. This leaves us with a system $\left(\rho',H'_S\right)$ with thermo-majorization curve identical to that of $\left(\rho,H_S\right)$ and such that:
\begin{equation}
\eta'_j e^{\beta E'_j}=\eta'_l e^{\beta E'_l},
\end{equation}
(i.e. the elbow defined in Eq. \eqref{eq:exact PF elbow} has moved to another part of the curve).

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/pf_1.pdf}
  \centerline{(a) Initial state.}
  \label{fig:PF initial}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figures/pf_2.pdf}
  \centerline{(b) Final state.}
  \label{fig:PF final}
\end{minipage}
\caption{\emph{Exact \longPF} Here we illustrate how to move a non-elbow point through the elbow, taking it from the left-hand segment to the right-hand one. First, we perform an \longITR\ that sends the non-elbow (triangle) towards the elbow (circle) while keeping it in thermal equilibrium with the left-hand segment. As the appropriate energy level is raised to infinity during the protocol, the triangle tends towards the circle until they coincide. Next, a second \longITR\ lowers the energy level from infinity while keeping it in thermal equilibrium with the right-hand part of the curve. This gives us a non-elbow point on the right-hand segment.}
\label{fig:exact PF}
\end{figure}


Exact \longPF\ requires that an energy level is raised to infinity during an \longITR. If it is not possible, or undesirable, to raise an energy level to infinity, a similar effect to an Exact \longPF\ can be achieved while altering the shape of the thermo-majorization curve slightly in a process we call \emph{Approximate \longPF}.
\begin{definition}[Approximate \longPF\ (A\PF)]
Approximate \longPF\ is illustrated in Figure \ref{fig:approximate PF}. Given an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ and state $\rho=\sum_{i=1}^{n} \eta_i\ketbra{i}{i}$ such that:
\begin{equation} \label{eq:approx PF elbow}
\eta_j e^{\beta E_j}=\eta_k e^{\beta E_k},
\end{equation}
for some $j,k$ (i.e. there is a non-elbow point on the thermo-majorization curve), an Approximate \longPF\ moves this non-elbow to an adjacent segment of the thermo-majorization curve whilst modifying the shape of the thermo-majorization curve by an arbitrarily small amount and without sending an energy level to infinity.
\end{definition}

To implement it, without loss of generality, assume that the set $\left\{i\right\}_{i=1}^{n}$ has been $\beta$-ordered, we wish to move the non-elbow point to the right and take $j=k+1$. To do this, we:
\begin{enumerate}
\item Apply a \ITR\ that raises the energy level of $E_j$ to some fixed, large but finite amount. This lowers the energy of $E_k$ and does not alter the shape of the thermo-majorization curve.
\item We now apply:
\begin{equation}
\textrm{\PLT}_{\left\{j,j+1\right\}}\left(\lambda=1\right),
\end{equation}
to the system. This turns the non-elbow associated with $j$ and $k$ into an elbow and the elbow associated with $j$ and $j+1$ into a non-elbow.
\item Using a \ITR, we can now move the new non-elbow point without altering the shape of the thermo-majorization curve.
\end{enumerate}
(i.e. the elbow defined in Eq. \eqref{eq:exact PF elbow} has moved to another part of the curve). By adjusting the height to which $E_j$ is raised in Step 1, we can tune the extent to which the thermo-majorization curve is altered.

\begin{figure}[h]
\begin{center}
$
\begin{array}{ccccc}
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/pf_general} & \qquad
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/pf1_general} \\
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/pf2_general}& \qquad
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/pf3_general}\\
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/pf4_general}
\end{array}
$
\end{center}
\caption{\emph{Approximate \longPF.} Here we illustrate the protocol of Approximate \longPF\ using thermo-majorization diagrams. Initially the system is as per Figure a). Using a \ITR, Figure b), the non-elbow point 1, is moved towards the elbow at point 2. This results in Figure c). Next, a \PLT\ is applied between points 1 and 3, Figure c), resulting in Figure d). Point 2 is now a non-elbow and can be moved using a \ITR, Figure e).}
\label{fig:approximate PF}
\end{figure}






\newpage

\section{State transformations when the Hamiltonian in trivial} \label{sec:transforms}


\begin{figure}[h]
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/disillation-boxes}
  \label{fig:Dist}
	\caption{Blah blah distillation}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{figures/formation-boxesf}
  \label{fig:Form}
	\caption{blah blah formation}
\end{minipage}


\caption{\emph{Deterministic work extraction, formation, and arbitrary transformations when H=0} Here we illustrate the protocol of}
\label{fig:boxes D&F}

\end{figure}


\begin{figure}[h]
\begin{center}
$
\begin{array}{cc}
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/disillation-boxes} & \qquad
\includegraphics[width=0.4\textwidth, height=0.311\textheight]{figures/formation-boxes}
\end{array}
$
\end{center}
\caption{\emph{Deterministic work extraction, formation, and arbitrary transformations when H=0} Here we illustrate the protocol of}
\label{fig:boxes}
\end{figure}


\section{States with same $\beta$-order} \label{sec:same order}

In this appendix, we show that for two states with the same $\beta$-ordering, if one thermo-majorizes the other, then the transition can be made using a finite number of \longPLTs. Furthermore, these \longPLTs\ need only act on two energy levels at a time.

We say that two states $\rho$ and $\sigma$, associated with the same Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$, have the same $\beta$-ordering if:
\begin{equation}
\sum_{i=1}^{k} e^{-\beta E^{\left(\rho\right)}_i} = \sum_{i=1}^{k} e^{-\beta E^{\left(\sigma\right)}_i}, \quad\forall k.
\end{equation}

\begin{theorem} \label{th:same beta order}
Suppose that $\rho$ and $\sigma$ are states of an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ such that:
\begin{enumerate}
\item $\sigma$ is block-diagonal in the energy eigenbasis.
\item $\rho$ and $\sigma$ have the same $\beta$-order.
\item $\rho$ thermo-majorizes $\sigma$.
\end{enumerate}
Then $\rho$ can be converted into $\sigma$ using at most $n-1$ \longPLTs.
\end{theorem}
\begin{proof}
To prove this, we give a protocol consisting only of \longPLTs\ that converts $\rho$ into $\sigma$. An illustrative outline for the protocol is given in Figure \ref{fig:SBO}. As we can perform any energy conserving unitary on the system, we can assume that both $\rho$ and $\sigma$ are diagonal in the energy eigenbasis (by decohering $\rho$ if necessary).

Let $\left\{\eta_i\right\}_{i=1}^{n}$ be the $\beta$-ordered eigenvalues of $\rho$, $\left\{\zeta_i\right\}_{i=1}^{n}$ be the $\beta$-ordered eigenvalues of $\sigma$ and $\left\{E_i\right\}_{i=1}^{n}$ be the $\beta$-ordered energy-eigenvalues of $H_S$.

Given that $\rho$ and $\sigma$ have the same $\beta$-order, $\rho$ majorizes $\sigma$ if and only if:
\begin{equation} \label{eq:majorization1}
\sum_{i=1}^{m} \eta_i \geq \sum_{i=1}^{m} \zeta_i, \quad \forall m.
\end{equation}
Let $\mathcal{M}$ be the set of $m$ for which equality occurs in Eq.~\eqref{eq:majorization1}. Suppose that are $r$ of them, and label them in ascending order by $\left\{t_s\right\}_{s=1}^{r}$. Note that $t_r=n$ and for convenience, define $t_0=0$.

We now proceed to perform a \PLT\ on each set of energy levels $\mathcal{P}^s\equiv\left\{t_{s-1}+1,\dots,t_{s}\right\}$ for $1\leq s\leq r$. For each $m\in\mathcal{P}^s$, let $\lambda^s_m$ be defined as the solution to:
\begin{equation}
\sum_{j=t_{s-1}+1}^{m}\left[ \left(1-\lambda^s_m\right)\eta_j+\frac{\lambda^s_m e^{-\beta E_j}}{\sum_{l\in\mathcal{P}^s}e^{-\beta E_l}}\sum_{l\in\mathcal{P}^s}\eta_l\right]=\sum_{j=t_{s-1}+1}^{m} \zeta_j,
\end{equation}
i.e. $\lambda^s_m$ is such that if one were to apply $\textrm{PT}_{\mathcal{P}^s}\left(\lambda^s_m\right)$ to $\rho$, the thermo-majorization curve of the resultant state would touch or cross the thermo-majorization curve of $\sigma$ at $m$. To ensure the resultant state thermo-majorizes $\sigma$, we actually apply the transformation $\textrm{PT}_{\mathcal{P}^s}\left(\lambda^s_{\textrm{min}}\right)$ for each $s$ where:
\begin{equation}
\lambda^s_{\textrm{min}}=\min_{m\in\left\{t_{s-1}+1,\dots,t_{s}\right\}} \lambda^s_m.
\end{equation}
This leaves us with a state $\rho'$ that has the same $\beta$-ordering as $\rho$ and $\sigma$ and thermo-majorizes $\sigma$.

Let $\left\{\eta'_i\right\}_{i=1}^{n}$ be the $\beta$-ordered eigenvalues of $\rho'$. Then $r'$, the number of $m$ such that:
\begin{equation}
\sum_{i=1}^{m} \eta'_i = \sum_{i=1}^{m} \zeta_i,
\end{equation}
is greater than or equal to $r$ with equality if and only if $r=n$. Hence by iterating the above procedure at most $n-1$ times, we transform $\rho$ into $\sigma$ using \longPLTs.
\end{proof}
\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/SBO1Graph.pdf}
  \label{fig:SBO1}
	\centerline{(a) First \PLT}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/SBO2Graph.pdf}
  \label{fig:SBO2}
	\centerline{(b) Second \PLT}
\end{minipage}\\
\vspace{.5cm}
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/SBO3Graph.pdf}
  \label{fig:SBO3}
	\centerline{(c) Final PLT}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{article_figures/SBO4Graph.pdf}
  \label{fig:SBO4}
	\centerline{(d) Final state, $\sigma$}
\end{minipage}
\caption{\emph{\longCOs\ protocol for transforming between states with the same $\beta$-order.} If two states, $\rho$ and $\sigma$, have the same $\beta$-order and are such that $\rho$ thermo-majorizes $\sigma$, then $\rho$ can be converted into $\sigma$ using \longPLTs. First a \PLT\ is applied to $\rho$ across the complete set of the energy levels, Figure (a), lowering the thermo-majorization of $\rho$ until it meets that of $\sigma$, Figure (b). Next, a second \PLT\ is applied to those energy levels to the left of this meeting point, again lowering the curve until it meets that of $\sigma$ at a second point, Figure (c). By iterating this process, $\rho$ is transformed into $\sigma$, Figure (d).}
\label{fig:SBO}
\end{figure}

%Original Figure
%\begin{figure}[h]
%\begin{center}
%$
%\begin{array}{cccc}
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_1} & \qquad
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_2} \\
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_3}& \qquad
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_4}\\
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_5}& \qquad
%\includegraphics[width=0.4\textwidth, height=0.3\textheight]{figures/cascades_6}\\
%\end{array}
%$
%\end{center}
%\caption{\emph{Protocol for converting states with the same $\beta$-order.} Here we illustrate the protocol given in Theorem \ref{th:same beta order}. Figure a) The state $\rho$ (blue) thermo-majorizes the state $\sigma$ (green) and has the same $\beta$-order. Initially a \PLT\ parametrized by $\lambda$ is applied to the whole system. The value of $\lambda$ chosen is calculate, Figures b) and c), such that the resultant states thermo-majorization curve meets the curve of $\sigma$ at one point. This is Point 2 in Figure d) which shows the resultant state. The process is repeated, Figure e), finally resulting in $\rho$ being transformed into $\sigma$, Figure f).}
%\label{fig:same order}
%\end{figure}

\longPLTs\ that act on 2 energy levels at a time are analogous to the concept of $T$-transforms (see, for example, \cite[Chapter 2, Section B]{marshall2010inequalities}) in majorization theory. Within majorization theory, it is know that if the vector $\vec{v}$ majorizes $\vec{u}$, then $\vec{v}$ can be converted into $\vec{u}$ using a finite number of $T$-transforms \cite{muirhead1902some,hardy1952inequalities}. The equivalent result for thermo-majorization is captured in the following theorem:
\begin{theorem}
Suppose that $\rho$ and $\sigma$ are states of an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ such that:
\begin{enumerate}
\item $\sigma$ is block-diagonal in the energy eigenbasis.
\item $\rho$ and $\sigma$ have the same $\beta$-order.
\item $\rho$ thermo-majorizes $\sigma$.
\end{enumerate}
Then $\rho$ can be converted into $\sigma$ using at most $n-1$ \longPLTs\ that each act on 2 energy levels.
\end{theorem}
\begin{proof}
The aim is to construct a protocol consisting of such \PLTs\ that converts $\rho$ into $\sigma$. To do this, we perform a sequence of \PLTs. Each \PLT\ adjusts the gradients of two line-segments of the thermo-majorization curve of $\rho$ until one of them matches the gradient of the corresponding segment on $\sigma$. By picking the segments of $\rho$ such that one has gradient strictly greater than the corresponding segment on $\sigma$ and one has gradient strictly less than the corresponding segment on $\sigma$ this can always be done. Once all of the gradients have been matched, $\rho$ has been converted into $\sigma$. The full details of the protocol are below.
{\color{red}Again, by first decohering $\rho$ in the energy eigenbasis if necessary, we can assume that $\rho$ and $\sigma$ are diagonal in the energy eigenbasis.}

Let $\left\{\eta_i\right\}_{i=1}^{n}$ be the $\beta$-ordered eigenvalues of $\rho$, $\left\{\zeta_i\right\}_{i=1}^{n}$ be the $\beta$-ordered eigenvalues of $\sigma$ and $\left\{E_i\right\}_{i=1}^{n}$ be the $\beta$-ordered energy-eigenvalues of $H_S$. Hence we have:
\begin{align}
\eta_1 e^{\beta E_1}\geq\dots\geq\eta_n e^{\beta E_n},
\end{align}
and
\begin{align}
\zeta_1 e^{\beta E_1}\geq\dots\geq\zeta_n e^{\beta E_n}.
\end{align}
Given that $\rho$ and $\sigma$ have the same $\beta$-order, $\rho$ majorizes $\sigma$ if and only if:
\begin{equation} \label{eq:majorization}
\sum_{i=1}^{m} \eta_i \geq \sum_{i=1}^{m} \zeta_i, \quad \forall m.
\end{equation}

Let $j$ be the largest index such that $\eta_j e^{\beta E_j} > \zeta_j e^{\beta E_j}$ and $k$ be the smallest index larger than $j$ such that $\eta_k e^{\beta E_k} < \zeta_k e^{\beta E_k}$. This picks the segments we shall apply the \PLT\ to. Then:
\begin{equation} \label{eq:jk order}
\eta_j e^{\beta E_j}>\zeta_j e^{\beta E_j}\geq\zeta_k e^{\beta E_k}>\eta_k e^{\beta E_k},
\end{equation}
and note that $\eta_i=\zeta_i$ for $j<i<k$.

We now determine the amount that we need to thermalize by in order to transform the gradient of one of the segments of $\rho$ to that of $\sigma$. Define $\lambda_1$ to be the value of $\lambda$ such that:
\begin{equation}
\left(1-\lambda_1\right)\eta_j e^{\beta E_j} + \frac{\lambda_1\left(\eta_j+\eta_k\right)}{e^{-\beta E_j}+e^{-\beta E_k}}=\zeta_j e^{\beta E_j},
\end{equation}
and $\lambda_2$ to be such that:
\begin{equation}
\left(1-\lambda_2\right)\eta_k e^{\beta E_k} + \frac{\lambda_2\left(\eta_j+\eta_k\right)}{e^{-\beta E_j}+e^{-\beta E_k}}=\zeta_k e^{\beta E_k}.
\end{equation}
Note that:
\begin{equation}
\eta_j e^{\beta E_j}\geq\frac{\eta_j+\eta_k}{e^{-\beta E_j}+e^{-\beta E_k}}\geq\eta_k e^{\beta E_k},
\end{equation}
and hence $\lambda_1,\lambda_2\geq0$. Also, at least one of $\frac{\left(\eta_j+\eta_k\right)}{e^{-\beta E_j}+e^{-\beta E_k}} \leq \zeta_j e^{\beta E_j }$ or $\frac{\left(\eta_j+\eta_k\right)}{e^{-\beta E_j}+e^{-\beta E_k}} \geq \zeta_k e^{\beta E_k }$ holds as $\zeta_j e^{\beta E_j}\geq\zeta_k e^{\beta E_k}$. Hence at least one of $\lambda_1$ and $\lambda_2$ must lie in the interval $\left[0,1\right]$. Let:
\begin{equation}
\lambda=\min\left\{\lambda_1,\lambda_2\right\}.
\end{equation}

Let $\rho'$ be the state formed by applying the 2-level \longPLT\ $\textrm{\PLT}_{\left\{j,k\right\}}\left(\lambda\right)$ to $\rho$. Note that $\rho'$ has the same $\beta$-order as $\rho$ and $\sigma$. To see this, let $\left\{\eta'_i\right\}_{i=1}^{n}$ be the eigenvalues of $\rho'$ listed according to the $\beta$ ordering of $\rho$. Then:
\begin{align*}
\eta'_i&=\eta_i, \quad\textrm{for }1\leq i<j,\\
\eta'_i&=\zeta_i, \quad\textrm{for }j<i<k,\\
\eta'_i&=\eta_i, \quad\textrm{for }k< i<n,
\end{align*}
as the \longPLT\ does not change the occupation probabilities associated with $i\notin\left\{j,k\right\}$. Without loss of generality, suppose $\lambda=\lambda_1$ . Then $\eta'_j=\zeta_j$ and using Eq.~\eqref{eq:jk order} where appropriate, it is easy to see that:
\begin{equation}
\eta'_i e^{\beta E_i}\geq \eta'_{i+1} e^{\beta E_{i+1}}, \quad\textrm{for both }i\in\left\{1,\dots,k-2\right\} \textrm{ and }i\in\left\{k,\dots,n\right\}.
\end{equation}
To see that $\eta'_{k-1} e^{\beta E_{k-1}}\geq\eta'_{k} e^{\beta E_{k}}$, note that:
\begin{equation}
\eta'_{k} e^{\beta E_{k}}=\left(1-\lambda_1\right)\eta_k e^{\beta E_k} + \frac{\lambda_1\left(\eta_j+\eta_k\right)}{e^{-\beta E_j}+e^{-\beta E_k}}\leq\zeta_k e^{\beta E_k}\leq\zeta_{k-1} e^{\beta E_{k-1}}=\eta'_{k-1} e^{\beta E_{k-1}}.
\end{equation}
Hence the $\beta$-order of $\rho'$ is the same as $\rho$.

As \longPLT\ is a thermal operation, $\rho$ thermo-majorizes $\rho'$. Similarly, $\rho'$ thermo-majorizes $\sigma$. To see this, it suffices to show that Eq. \eqref{eq:majorization} still holds if we replace $\rho$ with $\rho'$. As $\eta_j+\eta_k=\eta'_j+\eta'_k$, this obviously holds for $m<j$ and $m\geq k$. By observing that $\eta'_j\geq\zeta_j$ the remaining cases follow.

Applying the procedure once, sets at least one of the occupation probabilities to that of $\sigma$. Hence, by repeating the procedure at most $n-1$ times, starting each iteration with the output of the previous \longPLT, we obtain $\sigma$. 
\end{proof}

\newpage
\section{\longPLTs\ and \longLTs\ are not sufficient} \label{sec:nogo}

In this appendix, we show that \longPLTs\ and \longLTs\ are not sufficient for implementing all transformations allowed under thermal operations.

\chris{Qubit counterexample needs to go here.}

\newpage

\section{States with different $\beta$-order}

In this appendix, we show that using the full set of \longCOs\ enables one to perform all transformations {\color{red}to block-diagonal states} allowed under thermal operations.

Whilst \longPLTs\ and \longLTs\ alone are not enough to perform a transformation allowed under thermal operations, by combining them with the ability to append a single ancillary system with known Hamiltonian in the Gibbs state, they become more powerful. Indeed, they can be used to perform any transition between block-diagonal states allowed under thermal operations without the need to expend any work. This is captured and proven in the following theorem:
\begin{theorem} \label{th:crude protocol with infty}
Suppose that $\rho$ and $\sigma$ are %block-diagonal
 states of an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ such that:
\begin{enumerate}
\item $\sigma$ is block-diagonal in the energy eigenbasis.
\item $\rho$ thermo-majorizes $\sigma$.
\end{enumerate}
Then $\rho$ can be converted into $\sigma$ using \longCOs\ without expending any work.
\end{theorem}
\begin{proof}
To prove this we give a protocol consisting only of: adding (and eventually discarding) an ancilla qubit, Exact \longPF\ protocols (as introduced in Definition \ref{def:EPF}) and \longPLTs. None of these operations cost work. By first decohering $\rho$ in the energy eigenbasis if necessary and using an energy conserving unitary to rotate $\sigma$, we can assume that both $\rho$ and $\sigma$ are diagonal in the energy eigenbasis.

Let $\left(\tau_A,H_A\right)$ denote the known ancilla qubit allowed under Operation 1 of \longCOs. The protocol then runs as follows:
\begin{align*}
\left(\rho,H_S\right)&\longrightarrow\left(\rho\otimes\tau_A,H_S+H_A\right)\\
&\stackrel{\textrm{E}\PF}{\longrightarrow}\left(\rho',H'_{SA}\right)\\
&\stackrel{\PLT}{\longrightarrow}\left(\sigma',H'_{SA}\right)\\
&\stackrel{\textrm{E}\PF}{\longrightarrow}\left(\sigma\otimes\tau_A,H_S+H_A\right)\\
&\longrightarrow\left(\sigma,H_S\right).
\end{align*}
Here $\left(\rho',H'_{SA}\right)$ is a system with the same thermo-majorization curve as $\left(\rho\otimes\tau_A,H_S+H_A\right)$. However, the non-elbow points have been moved (potentially while sending energy levels to infinity) so that on the thermo-majorization diagram, they are vertically in line with the elbows (including the point $(Z,1)$) of $\left(\sigma\otimes\tau_A,H_S+H_A\right)$. This transformation can be performed using E\PFs\ and \ITRs. 

Similarly, $\left(\sigma',H'_{SA}\right)$ is a system with the same thermo-majorization curve as $\left(\sigma\otimes\tau_A,H_S+H_A\right)$ but with the non-elbow points moved to lie vertically inline with the elbows of $\left(\rho\otimes\tau_A,H_S+H_A\right)$ and at $(Z,1)$. Again, this transformation can be performed (and reversed) using the \longPF\ protocol.

Note that by construction, $\left(\rho',H'_{SA}\right)$ has the same $\beta$-ordering as $\left(\sigma',H'_{SA}\right)$ and as $\rho$ thermo-majorizes $\sigma$, $\left(\rho',H'_{SA}\right)$ thermo-majorizes $\left(\sigma',H'_{SA}\right)$. Hence, by Theorem \ref{th:same beta order} it is possible to transform $\left(\rho',H'_{SA}\right)$ into $\left(\sigma',H'_{SA}\right)$ using \longPLTs.

The overall protocol is illustrated in Figure \ref{fig:DBO}.
\end{proof}
\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/DBO1Graph.pdf}
  \label{fig:DBO1}
	\centerline{(a) \ITRs\ and \PFs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/DBO2Graph.pdf}
  \label{fig:DBO2}
	\centerline{(b) Same $\beta$-order protocol applied}
\end{minipage}\\
\vspace{.5cm}
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{article_figures/DBO3Graph.pdf}
  \label{fig:DBO3}
	\centerline{(c) \ITRs\ and \PFs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{article_figures/DBO4Graph.pdf}
  \label{fig:DBO4}
	\centerline{(d) Upon discarding $\tau_A$, the final state is $\sigma$}
\end{minipage}
\caption{\emph{\longCOs\ protocol for transforming between states with different $\beta$-orders.} If $\rho$ thermo-majorizes $\sigma$, then it is possible to transform $\rho$ into $\sigma$ using \longCOs. First, a thermal qubit, $\tau_A$, with known Hamiltonian is appended, Figure (a). Using \longITRs\, the blue circles on the thermo-majorization curve of $\rho\otimes\tau_A$ can be moved to be vertically aligned with the `elbows' on the curve for $\sigma\otimes\tau_A$. This forms the state $\rho'$, Figure (b), that has a thermo-majorization curve overlapping that of $\rho\otimes\tau_A$. Using the previously defined protocol for states with the same $\beta$-order, $\rho'$ can be converted into $\sigma'$, Figure (c), that has a thermo-majorization curve overlapping that of $\sigma\otimes\tau_A$. A final round of \ITRs\ converts $\sigma'$ into $\sigma\otimes\tau_A$, Figure (d), and upon discarding $\tau_A$ we obtain $\sigma$.}
\label{fig:DBO}
\end{figure}


The protocol described in the above theorem potentially requires that an energy level be raised to infinite energy. While this can be done at no work cost (provided it is performed infinitely slowly during the \longPF\ protocol), note that such a transition is not required if the thermo-majorization curves of $\rho$ and $\sigma$ do not cross.
\begin{theorem}
Suppose that $\rho$ and $\sigma$ are %block-diagonal
 states of an $n$-level system with Hamiltonian $H_S=\sum_{i=1}^{n} E_i \ketbra{i}{i}$ such that:
\begin{enumerate}
\item $\sigma$ is block-diagonal in the energy eigenbasis.
\item $\rho$ thermo-majorizes $\sigma$.
\item The thermo-majorization curves of $\rho$ and $\sigma$ meet only at $\left(0,0\right)$ and $\left(Z_S,1\right)$.
\end{enumerate}
Then $\rho$ can be converted into $\sigma$ using \longCOs, without expending any work and without the need to raise an energy level to infinity.
\end{theorem}
\begin{proof}
Here we sketch how to modify the protocol given in Theorem \ref{th:crude protocol with infty} to avoid needing to raise an energy level to infinity. Again we can assume that $\rho$ and $\sigma$ are diagonal in the energy eigenbasis. The new protocol runs as follows:
\begin{align*}
\left(\rho,H_S\right)\longrightarrow&\left(\rho\otimes\tau_A,H_S+H_A\right)\\
\stackrel{\stackrel{\textrm{A}\PF}{\PLT}}{\longrightarrow}&\left(\tilde{\rho},H_S+H_A\right)\\
\stackrel{\PLT}{\longrightarrow}&\left(\sigma\otimes\tau_A,H_S+H_A\right)\\
\longrightarrow&\left(\sigma,H_S\right).
\end{align*}
Here $\left(\tilde{\rho},H_S+H_A\right)$ is a system with a thermo-majorization curve such that each one of its points (both elbows and non-elbows) are vertically aligned with the points of $\left(\sigma\otimes\tau_A,H_S+H_A\right)$.

To create $\left(\tilde{\rho},H_S+H_A\right)$, we use the following process, illustrated in Figure \ref{fig:ABO}:
\begin{enumerate}
\item Using Approximate \longPFs, adjust the points of $\rho\otimes\tau_A$ to form $\rho'$ which has non-elbow points vertically aligned with the elbows of $\sigma\otimes\tau_A$. There are $n-1$ such points. As the thermo-majorization curves of $\rho\otimes\tau_A$ and $\sigma\otimes\tau_A$ touch only at $(0,0)$ and at $\left(Z_S Z_A,1\right)$, the A\PF\ can be chosen such that $\rho'$ has the desired alignment, thermo-majorizes $\sigma\otimes\tau_A$ and such that the thermo-majorization curves of $\rho'$ inherits these properties.
\item For each vertically aligned point $i\in\left\{1,\dots n-1\right\}$ on $\rho'$, consider the number of points (both elbows and non-elbows) to the left of it on its thermo-majorization curve. Call this number $r_i$. Compare this quantity to the number of points to the left of the associated vertically aligned point on the thermo-majorization curve of $\sigma\otimes\tau_A$. Call this number $s_i$. If:
\begin{enumerate}
\item $r_i<s_i$: Move the point slightly to the right of its aligned location using a \ITR.
\item $r_i>s_i$: Move the point slightly to the left of its aligned location using a \ITR.
\item $r_i=s_i$: Leave the point where it is.
\end{enumerate}
These \ITRs\ result in a state $\rho''$ with the same thermo-majorization curve as $\rho'$.
\item Defining $i=0$ to be the point $(0,0)$ and $i=n$ to be the point $\left(Z_S Z_A,1\right)$, for each $i\in\left\{1,\dots n\right\}$ thermalize $\rho''$ over the the interval between points $i-1$ and $i$ using \PLTs.
This results in a state $\rho'''$ which has elbows almost vertically aligned with the elbows of $\sigma\otimes\tau_A$.
%This results in a state $\rho'''$ which has elbows in the same position as the non-elbows of $\rho''$ and non-elbows vertically aligned with the elbows of $\rho''$. 
Provided the movements due to \ITRs\ in Step 2 were chosen to be sufficiently small, as $\rho''$ thermo-majorizes $\sigma\otimes\tau_A$ and their thermo-majorization curves touch only at $(0,0)$ and $\left(Z_S Z_A,1\right)$, $\rho'''$ inherits the same properties.
\item Using Approximate \longPFs, adjust the points of $\rho'''$ to form $\tilde{\rho}$ as defined above. The last time an A\PF\ is applied to an elbow, it should be done in such a way that after the operation, the elbow is precisely vertically aligned with that of $\sigma\otimes\tau_A$. The displacements applied in Step 2 enable this to take place. As $\rho'''$ thermo-majorizes $\sigma\otimes\tau_A$ and their thermo-majorization curves touch only at (0,0) and $\left(Z_S Z_A,1\right)$, $\tilde{\rho}$ again inherits these properties. 
\end{enumerate}

Due to the fact that the protocol uses Approximate \longPFs\ rather than Exact \longPFs, there is no need to raise an energy level to infinity.

As $\left(\tilde{\rho},H_S+H_A\right)$ thermo-majorizes $\sigma\otimes\tau_A$ and they have the same $\beta$-ordering, the transformation can now be completed using \longPLTs\ as described in Theorem \ref{th:same beta order}.
\end{proof}

Note that there are scenarios in which the restriction that the curves touch only at $\left(0,0\right)$ and $\left(Z_S,1\right)$ in the above theorem can be relaxed slightly to demanding that the curves touch only at $\left(0,0\right)$ and on the line $y=1$. For example, this is the case if $\left|W_{\rho\rightarrow\tau_S}\right|>\left|W_{\sigma\rightarrow\tau_S}\right|$, where $\tau_S$ is the Gibbs state of the system's Hamiltonian, i.e. it is possible to extract strictly more work deterministically from $\rho$ than from $\sigma$. In general, allowing the curves to touch at $y=1$ makes the theorem more relevant for situations where we wish to model a change of Hamiltonian or include a work storage system as per Appendix \ref{ssec:wits&switch}.

\begin{figure}[h!]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO1.pdf}
  \centerline{(a) Initial state. Step 1: A\PFs.}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO2.pdf}
  \centerline{(b) Step 2: \ITRs.}
\end{minipage}\\
\vspace{1.7cm}
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO3.pdf}
  \centerline{(c) Step 3: \PLTs.}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO4.pdf}
  \centerline{(d) Step 4: A\PFs.}
\end{minipage}\\
\vspace{1.7cm}
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO5.pdf}
  \centerline{(e) Step 4: A\PFs\ continued.}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO6.pdf}
  \centerline{(f) Step 4: A\PFs\ continued.}
\end{minipage}
\end{figure}

\begin{figure}[h!]
\ContinuedFloat
\begin{flushleft}
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{supplementary_figures/ABO7.pdf}
  \centerline{(g) Final state with the same $\beta$-ordering as $\sigma\otimes\tau_A$.}
\end{minipage}
\end{flushleft}
\caption[$\beta$-order change with Approximate \longPFs.]{\emph{$\beta$-order change with Approximate \longPFs.} In Step 1 of the protocol, A\PFs\ are performed so that the non-elbows of $\rho\otimes\tau_A$ can be horizontally aligned with the elbows of $\sigma\otimes\tau_A$. This transforms Figure (a) into Figure (b). In Step 2, \ITRs\ are used to slightly misaligned the points in anticipation of Step 4. In this example they are misaligned to the right resulting in Figure (c). Next, \PLTs\ are used in Step 3 to generate elbows (almost) horizontally aligned with those of $\sigma\otimes\tau_A$. This leads to Figure (d). Finally, in Step 4 A\PFs\ are applied to exactly match the elbows together with the non-elbow points. This is detailed in Figures (e) and (f). The result of the protocol is shown in Figure (g).}
\label{fig:ABO}
\end{figure}



\newpage


\section{Quantifying worst-case work costs with \longCOs}

Instead of using the wit construction summarized in Section \ref{ssec:wits&switch} to analyze the work costs of a transformation, under \longCOs\ one can consider the cost of \longLTs\ as defined in Eq.~\eqref{eq:LT cost}. In this section, we shall that using this approach reproduces the results regarding worst-case work obtained under noisy operations in \cite{horodecki2013fundamental}.

\subsection{Extractable work} \label{ss:extractwork}

%\chris{Protocol extracts work less than Aaberg and TO case by an additive faction of $\frac{1}{\beta}\ln\left(1-\epsilon\right)$. This seems better than allowing a measurement (which would introduce a $\ln2$ factor) and doesn't cost infinite work in the event of a failure. Not sure whether this is worth including or if we should stick to deterministic ($\epsilon=0$) work or reproduce Aaberg and not worry about the infinity.}

By setting the final state to be $\tau_S$, the thermal state of the system, in Eq. \eqref{eq:work def}, one can define the single-shot \emph{distillable work} - the amount of work that can be obtained from a state. One can also consider the \emph{smoothed} distillable work, where one allows the possibility of failing to distil positive work with some probability $\epsilon$. Denoting this quantity for a given state $\rho$ by $W^{\epsilon}_{\textrm{form}}\left(\rho\right)$, in \cite{horodecki2013fundamental, aaberg2013truly} it was shown to be given by:
\begin{align}
\begin{split} \label{eq:distill work}
W^{\epsilon}_{\textrm{distil}}\left(\rho\right)&=F_{\textrm{min}}^{\epsilon}\left(\rho\right)+\frac{1}{\beta}\ln Z\\
&=-\frac{1}{\beta} \left[\ln\left(\tilde{L}_{1-\epsilon}\left(\rho\right)\right)-\ln Z\right],
\end{split}
\end{align}
where $\tilde{L}_{y}$ denotes the horizontal distance between a state's thermo-majorization curve and the $y$-axis at $y$, a quantity discussed more fully in \cite{alhambra2015probability}.

In Figure \ref{fig:Abergs protocol} we represent using thermo-majorization diagrams the protocol from \cite{aaberg2013truly} that distills the amount of work given in Eq.~\eqref{eq:distill work} using \longCOs. {\color{red}As decohering is a crude operation which commutes with all other thermal operations, we can first decohere $\rho$ without altering the amount of work we can extract.} Let $Z_\epsilon=\tilde{L}_{1-\epsilon}\left(\rho\right)$ denote the point on the $x$-axis such that those energy levels to the left of it on the thermo-majorization curve of $\rho$ have cumulative population given by $1-\epsilon$ and those energy levels to the right have total weight $\epsilon$. Note that without loss of generality we can assume that $\left(Z_\epsilon,1-\epsilon\right)$ is either an elbow or non-elbow on the thermo-majorization curve of $\rho$ as we can always make it so by appending a qubit ancilla $\tau_A$, considering the thermo-majorization curve of $\rho\otimes\tau$ and preceding the extraction protocol with a \longITR\ to move a non-elbow to the desired location.

The protocol runs as follows:
\begin{enumerate}
\item Raise the energy levels to the right of $Z_\epsilon$ to infinity using \longLTs.
\item Fully thermalize the system.
\item Perform \longITRs\ to horizontally align the points on the system's thermo-majorization curve with those of the target thermal state.
\item Perform a \longLT\ to transform the system into the thermal state of the initial Hamiltonian.
\end{enumerate}
Two stages of this protocol cost/yield work. The \longLT\ that takes Figure \ref{fig:Abergs protocol}(a) to Figure \ref{fig:Abergs protocol}(b) costs an infinitely large amount of work with probability $\epsilon$ and no work with probability $1-\epsilon$. The second \longLT\ that takes Figure \ref{fig:Abergs protocol}(c) to Figure \ref{fig:Abergs protocol}(d), has deterministic work yield $\frac{1}{\beta}\ln\left(\frac{Z}{Z_\epsilon}\right)$. Hence the overall protocol achieves the work cost given in Eq.~\eqref{eq:distill work}. \chris{Do we want to add some more here about how the TO protocol avoids the infinite work cost upon failure?}
 
\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtractB1.pdf}
  \label{fig:ExtractB1}
	\centerline{(a) \LTs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtractB2.pdf}
  \label{fig:ExtractB2}
	\centerline{(b) \PLTs}
\end{minipage}\\
\vspace{.5cm}
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtractB3.pdf}
  \label{fig:ExtractB3}
	\centerline{(c) \ITRs\ and \LTs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{supplementary_figures/ExtractB4.pdf}
  \label{fig:ExtractB4}
	\centerline{(d) Final state, $\tau$}
\end{minipage}
\caption{\emph{\longCOs\ protocol for $\epsilon$-deterministic work extraction.} Here we illustrate the protocol for $\epsilon$-deterministic work extraction from \cite{aaberg2013truly} in terms of thermo-majorization diagrams. Note that the first step, transforming Figure (a) into Figure (b), involves raising energy levels to infinity. This costs an infinitely large amount of work with probability $\epsilon$ and no work with probability $1-\epsilon$. Energy levels can instead be raised to some large but finite energy (for finite work cost) at the expense of extracting less work during the \longLTs\ that transform Figure (c) into Figure (d).} \label{fig:Abergs protocol}
\end{figure}

However, when this protocol fails, it fails spectacularly and costs an infinitely large amount of work. As discussed in \cite{aaberg2013truly}, this can be avoided if, instead of raising energy levels to infinity during the first \longLT, we instead raise them to a large but finite amount. However, this reduces the amount of work that is extracted when the protocol succeeds. The tradeoff between the cost of failure and the benefit of success is analyzed through the protocol given in Figure \ref{fig:finite extract protocol}.

Let $V$ denote the amount of work we are willing to expend to raise the energy levels to the right of $Z_\epsilon$ (as we are raising energy levels, $V$ is negative). The protocol then runs as follows:
\begin{enumerate}
\item Raise the unoccupied energy levels to the right of $Z_\epsilon$ to infinity using \longLTs.
\item Raise the occupied energy levels to the right of $Z_\epsilon$ by the amount $V$ using \longLTs.
\item Fully thermalize the entire system.
\item Perform \longITRs\ to horizontally align the points on the system's thermo-majorization curve with those of the target thermal state.
\item Perform a \longLT\ to transform the system into the thermal state of the initial Hamiltonian.
\end{enumerate}
Again, two stages of this protocol cost/yield work. The \longLT\ that takes Figure \ref{fig:finite extract protocol}(a) to Figure \ref{fig:finite extract protocol}(b) costs an amount of work given by $V$ with probability $\epsilon$ and no work with probability $1-\epsilon$. The second \longLT that takes Figure \ref{fig:finite extract protocol}(c) to Figure \ref{fig:finite extract protocol}(d), has deterministic work yield $\frac{1}{\beta}\ln\left(\frac{Z}{Z_\epsilon+e^{\beta V}\left(\tilde{L}_{1}\left(\rho\right)-Z_\epsilon\right)}\right)$. Hence, with probability $1-\epsilon$ the protocol produces a work gain of:
\begin{equation}
\frac{1}{\beta}\ln\left(\frac{Z}{Z_\epsilon+e^{\beta V}\left(\tilde{L}_{1}\left(\rho\right)-Z_\epsilon\right)}\right),
\end{equation}
while with probability $\epsilon$ it costs work:
\begin{equation}
\frac{1}{\beta}\ln\left(\frac{Z}{Z_\epsilon+e^{\beta V}\left(\tilde{L}_{1}\left(\rho\right)-Z_\epsilon\right)}\right)+V.
\end{equation}
As $V$ tends to negative infinity, we recover Eq.~ \eqref{eq:distill work} while when $V=0$, the amount of work extracted is equal to $W^{0}_{\textrm{form}}\left(\rho\right)$.

\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtV1.pdf}
  \label{fig:ExtractV1}
	\centerline{(a) \LTs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtV2.pdf}
  \label{fig:ExtractV2}
	\centerline{(b) \PLTs}
\end{minipage}\\
\vspace{.5cm}
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/ExtV3.pdf}
  \label{fig:ExtractV3}
	\centerline{(c) \longITRs\ and \longLTs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{supplementary_figures/ExtV4.pdf}
  \label{fig:ExtractV4}
	\centerline{(d) Final state, $\tau$}
\end{minipage}
\caption{\emph{\longCOs\ protocol for $\epsilon$-deterministic work extraction without infinite cost upon failure.} Here we illustrate the protocol for $\epsilon$-deterministic work extraction without infinite work cost upon failure. Note that this protocol produces less work when it succeeds than that described in Figure \ref{fig:Abergs protocol}.} \label{fig:finite extract protocol}
\end{figure}

%In Figure \ref{fig:work extraction}, we give a protocol that distills the amount of work given by Eq.~\eqref{eq:distill work} (up to a $\ln\left(1-\epsilon\right)$ factor) with probability $1-\epsilon$. To see this, first define $x_\epsilon=\tilde{L}_{1-\epsilon}\left(\rho\right)$. Note that without loss of generality we can assume that $\left(x_\epsilon,1-\epsilon\right)$ is a point used for defining the thermo-majorization curve of $\rho$ (it belongs to the set defined in Eq.~\eqref{eq:th-maj set}). If it does not, by appending a thermal qubit and using a \longITR\, we can move a point on the thermo-majorization curve to this location. Note also that the \longPLTs\ and \longITRs\ shown in Figure \ref{fig:work extraction} cost no work.

%Consider now the two \longLTs. The first, that which takes Figure \ref{fig:work extraction}(b) to Figure \ref{fig:work extraction}(c), has associated work distribution:
%\begin{align}
%P\left(W=0\right)&=1-\epsilon,\\
%P\left(W=\frac{1}{\beta}\ln\left[\frac{\epsilon x_\epsilon}{\left(Z_S-x_\epsilon\right)\left(1-\epsilon\right)}\right]\right)&=\epsilon,
%\end{align}
%while the second, that which takes Figure \ref{fig:work extraction}(d) to Figure \ref{fig:work extraction}(e), has a deterministic work cost:
%\begin{equation}
%P\left(W=\frac{1}{\beta}\left[\ln Z_S+\ln\left(1-\epsilon\right)-\ln x_\epsilon\right]\right)=1.
%\end{equation}
%Hence the protocol distills work:
%\begin{equation}
%\frac{1}{\beta}\left[\ln Z_S+\ln\left(1-\epsilon\right)-\ln\left(\tilde{L}_{1-\epsilon}\right)\right],
%\end{equation}
%with probability $1-\epsilon$. Note that with probability $\epsilon$, the protocol costs work rather than distilling it. Note that in contrast to the protocol given in \cite{aaberg2013truly}, the protocol does not cost an arbitrarily large amount of work in the event that it fails. This is however at the expense of drawing $\ln\left(1-\epsilon\right)$ less work when it succeeds. 

%\begin{figure}
%\centering
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[width=0.9\textwidth]{supplementary_figures/Ext1Graph.pdf}
%  \label{fig:Ext1}
%	\caption{\longPLTs}
%\end{subfigure}%
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[width=0.9\textwidth]{supplementary_figures/Ext2Graph.pdf}
%  \label{fig:Ext2}
%	\caption{\longLTs}
%\end{subfigure}\\
%\vspace{.5cm}
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[width=0.9\textwidth]{supplementary_figures/Ext3Graph.pdf}
%  \label{fig:Ext3}
%	\caption{\longITRs}
%\end{subfigure}%
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[width=.9\textwidth]{supplementary_figures/Ext4Graph.pdf}
%  \label{fig:Ext4}
%	\caption{\longLTs}
%\end{subfigure}\\
%\vspace{.5cm}
%\begin{flushleft}
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[width=.9\textwidth]{supplementary_figures/Ext5Graph.pdf}
%  \label{fig:Ext5}
%	\caption{Final state, $\tau$}
%\end{subfigure}
%\end{flushleft}
%\caption{\emph{\longCOs\ protocol for $\epsilon$-deterministic work extraction.}} \label{fig:work extraction}
%\end{figure}


\subsection{Work of formation} \label{ss:formwork}

By setting the initial state to be $\tau_S$, the thermal state of the system, in Eq. \eqref{eq:work def}, one can define the single-shot \emph{work of formation} - the amount of work required to form a state without coherences. Denoting the work of formation for block-diagonal $\rho$ by $W_{\textrm{form}}\left(\rho\right)$, in \cite{horodecki2013fundamental} it was shown to be given by:
\begin{align}
\begin{split} \label{eq:work form}
W_{\textrm{form}}\left(\rho\right)&=-F_{\textrm{max}}\left(\rho\right)-\frac{1}{\beta}\ln Z_S,\\
&=-\frac{1}{\beta}\left[\ln\left(\eta^{\left(\rho\right)}_1 e^{\beta E_1^{\left(\rho\right)}}\right)+\ln Z_S\right].
\end{split}
\end{align}

In Figure \ref{fig:work of formation}, we give a protocol to form such a $\rho$ from the thermal state that has work cost given by Eq.~\eqref{eq:work form}. To see this, note that by Lemma \ref{le:ITR cost}, the work cost of the \longITRs\ can be made to be zero. Let the first \longLT, that which takes Figure \ref{fig:work of formation}(b) to Figure \ref{fig:work of formation}(c), be parametrized by $\mathcal{E}=\left\{h_i\right\}_{i=1}^{n}$ and the second \longLT, which takes Figure \ref{fig:work of formation}(c) to Figure \ref{fig:work of formation}(d), by $\mathcal{E}'=\left\{h'_i\right\}_{i=1}^{n}$. Here:
\begin{align}
h_i&=\frac{1}{\beta}\left[\ln\left(\eta^{\left(\rho\right)}_1 e^{\beta E_1^{\left(\rho\right)}}\right)+\ln Z_S\right], \quad \forall i,\\
h'_i&\leq0, \quad\forall i.
\end{align}
Hence:
\begin{align}
W_{\LT_{\mathcal{E}}}&=-\frac{1}{\beta}\left[\ln\left(\eta^{\left(\rho\right)}_1 e^{\beta E_1^{\left(\rho\right)}}\right)+\ln Z_S\right],\\
W_{\LT_{\mathcal{E}'}}&=0,
\end{align}
and the overall formation protocol has work cost given by Eq.~\eqref{eq:work form}.
\begin{figure}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/Form1Graph.pdf}
  \label{fig:Form1}
	\centerline{(a) \ITRs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/Form2Graph.pdf}
  \label{fig:Form2}
	\centerline{(b) \LTs}
\end{minipage}\\
\vspace{.5cm}
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{supplementary_figures/Form3Graph.pdf}
  \label{fig:Form3}
	\centerline{(c) \LTs}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{supplementary_figures/Form4Graph.pdf}
  \label{fig:Form4}
	\centerline{(d) Final state, $\rho$}
\end{minipage}
\caption{\emph{\longCOs\ protocol for state formation.}} \label{fig:work of formation}
\end{figure}

\subsection{Work of transformation}

Given two states, $\rho$ and $\sigma$, recall from Section \ref{ssec:wits} that $\Wtran{\rho}{\sigma}$ denotes the deterministic work required (if $\Wtran{\rho}{\sigma}$ is negative)  or gained (if $\Wtran{\rho}{\sigma}$ is positive) in converting $\rho$ into $\sigma$ using thermal operations. This quantity can readily be obtained under \longCOs. If one first performs the \longLT, $\LT_{\mathcal{E}}$ with $\mathcal{E}=\left\{h_i=\Wtran{\rho}{\sigma}\right\}_{i=1}^{n}$ to $\left(\rho,H_S\right)$ by definition, one is left with a system that thermo-majorizes $\left(\sigma,H_S\right)$. This system can now be converted into $\left(\sigma,H_S\right)$ using the protocol given in Theorem \ref{th:crude protocol with infty} and the work cost of the \LT\ is $\Wtran{\rho}{\sigma}$.

%\end{document}

==> Supplementary_Material/common/definitions.tex <==


%\def\wit{wit}
\def\toto{\mathop{\to}\limits^{TO}}
\def\pij{p_{i\to j}}
\def\dmin{D_{\min}}
\def\dmax{D_{\max}}
\def\<{\langle}
\def\>{\rangle}
\def\ot{\otimes}
\def\ermax{E_R^{\max}}
\def\esmax{E_S^{\max}}
\def\ecal{{\cal E}}
\def\hcal{{\cal H}}
\def\ecalr{{\ecal_R}}
\def\etaE{\eta_{E-E_S}^R}
\def\etaEprim{\eta'_{E-E_S}}
\def\ideta{\eta}
\def\rhor{\rho_R}
\def\rhos{\rho_S}
\def\rhors{\rho_{RS}}
\def\energy{E_0}

\def\rhoinr{\rho^{\rm in}_R}
\def\rhoins{\rho^{\rm in}_S}
\def\rhoinw{\rho^{\rm in}_W}
\def\rhoinc{\rho^{\rm in}_C}
\def\rhooutr{\rho^{\rm out}_R}
\def\rhoouts{\rho^{\rm out}_S}
\def\rhooutw{\rho^{\rm out}_W}
\def\rhooutsc{\rho^{\rm out}_{SC}}
\def\rhooutsw{\rho^{\rm out}_{SW}}
\def\rhooutc{\rho^{\rm out}_C}
\def\rhozeror{\rho^{0}_R}
\def\rhozeros{\rho^{0}_S}
\def\rhozeroc{\rho^{0}_C}
\def\sgibbs{\rho_S^\beta}
\def\rgibbs{\rho_R^\beta}
\def\cgibbs{\rho_C^\beta}
\def\ancgibbs{\rho_{\rm anc}^\beta}
\def\rscgibbs{\rho_{\rm RSC}^\beta}
\def\scgibbs{\rho_{\rm SC}^\beta}

\def\twirl{{\cal T}}
%\def\rk{{\rm rank}}
\def\tred{\textcolor{red}}
\def\tblue{\textcolor{blue}}
\def\funny{{f-smooth}}
\def\funnyh{{f-smooth}}
\def\Funnyh{{F-smooth}}
\def\fh{\tilde H}
\def\Funny{{F-smooth}}
\def\frk{{\rm{frk}}}
\def\ftail{{\rm{ftail}}}
\def\tail{{\rm tail}}
\def\rk{{\rm rk}}
\def\rkd{{\rm rk}^\delta}

\def\stipp{\bar{p}^{(\delta)}}
\def\stipq{\bar{q}^{(\delta)}}
\def\stipf{\bar{f}^{(\delta)}}
\def\flatp{\underline{p}^{(\delta)}}
\def\flatq{\underline{q}^{(\delta)}}
\def\flatf{\underline{f}^{(\delta)}}
\def\flattest{flattest}
\def\stippest{steeppest}




\newcommand{\be}{\begin{eqnarray} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{eqnarray} }
\newcommand{\benn}{\begin{eqnarray*} \begin{aligned}}
\newcommand{\eenn}{\end{aligned} \end{eqnarray*} }


\newcommand{\ben}{\begin{eqnarray} \begin{aligned}}
\newcommand{\een}{\end{aligned} \end{eqnarray} }

\newcommand{\hmax}{\mathrm{H}_{\max}}
\newcommand{\hminp}{\mathrm{H}_{\min}}
\newcommand{\h}{\mathrm{H}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\ran}{\rangle}
\newcommand{\lan}{\langle}
\newcommand{\id}{\mathbb{I}}
\newcommand{\im}{\mathbbmss{1}}
\newcommand{\idop}{\mathcal{I}}
\newcommand{\nullmat}{\mathbf{0}}
\newcommand{\fid}{\mathcal{F}}
\newcommand{\Cn}{\mathbb{C}}
\newcommand{\re}{\mathop{\mathbb{R}}\nolimits}
\newcommand{\natnum}{\mathop{\mathbb{N}}\nolimits}
\newcommand{\esp}{\mathbb{E}}
\newcommand{\cov}{\mathop{\mathrm{Cov}} \nolimits}
\newcommand{\var}{\mathop{\mathrm{Var}} \nolimits}
\newcommand{\mse}{\mathop{\mathrm{MSE}} \nolimits}
\newcommand{\rlprt}{\mathop{\mathrm{Re}} \nolimits}
\newcommand{\nth}{\mathrm{th}}
\newcommand{\imprt}{\mathop{\mathrm{Im}}\nolimits}
\newcommand{\tr}{\mathop{\mathsf{tr}}\nolimits}
\newcommand{\Tr}{\mathop{\mathsf{Tr}}\nolimits}
\newcommand{\eval}[2]{\left. #1 \right \arrowvert _{#2}}
\newcommand{\norm}[1]{\left\| #1\right \|}
\newcommand{\smalloh}{\mathrm{o}}
\newcommand{\bigoh}{\mathrm{O}}
\newcommand{\pr}{\prime}
\newcommand{\di}{\text{d}}
\newcommand{\trans}[1]{#1^{\top}}
\newcommand{\iu}{i}
\newcommand{\vc}[1]{#1}				% VECTORS
\newcommand{\abs}[1]{\left|#1 \right|}				% ABS
\newcommand{\der}[1]{\frac{\partial}{\partial #1}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\upa}{\uparrow}
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proposition}{Proposition}[section]
%MH
\newcommand{\beq}{\begin{eqnarray} \begin{aligned}}
\newcommand{\eeq}{\end{aligned} \end{eqnarray} }
\newcommand{\bea}{\begin{array}}
\newcommand{\eea}{\end{array}}


\newcommand{\bee}{\begin{enumerate}}
\newcommand{\eee}{\end{enumerate}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
%MH
\newtheorem{examp}[theorem]{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newcommand{\dna}{\downarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\hil}{\mathcal{H}}
\newcommand{\kil}{\mathcal{K}}
\newcommand{\allrhos}{\mathcal{M}}
\newcommand{\allrhosin}[1]{\mathcal{S}(#1)}
\newcommand{\pop}[1]{\mathcal{M}_{+}(#1)}
\newcommand{\cpmap}{\mathcal{E}}
\newcommand{\uop}{\mathcal{U}}
\newcommand{\su}{\mathfrak{su}}
\newcommand{\finproof}{$\Box$}
\newcommand{\textmath}{}
\newcommand{\wt}{\widetilde}
\newcommand{\wavyline}[3]{
\multiput(#1,#2)(4,0){#3}{
\qbezier(0,0)(1,1)(2,0)
\qbezier(2,0)(3,-1)(4,0)}}
\newcommand{\spann}{\mathop{\mathrm{span}}\nolimits}  %%% Space spanned by a set of vectors.



\newcommand{\wigglyline}[3]{
\multiput(#1,#2)(1,0){#3}{
\qbezier(0,0)(0.25,0.25)(0.5,0)
\qbezier(0.5,0)(0.75,-0.25)(1,0)}}

\newcommand{\allsigmasin}[1]{\tilde{\mathcal{S}}(#1)}
\newcommand{\instr}{\mathcal{N}}
\newcommand{\dfdas}{\stackrel{\textrm{\tiny def}}{=}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\nolimits}
\newcommand{\bin}{\textrm{Bin}}
\newcommand{\topr}{\stackrel{P}{\to}}
\newcommand{\todst}{\stackrel{D}{\to}}
\newcommand{\lil}{\mathcal{L}}
\newcommand{\myabstract}[1]{\begin{quote}{\small  #1 }\end{quote}}
\newcommand{\myacknowledgments}{\begin{center}{\bf Acknowledgments}\end{center}\par}
\newcommand{\otherfid}{\mathsf{F}}
\newcommand{\mypacs}[1]{\begin{flushleft} {\small PACS numbers: #1}\end{flushleft}}
\newcommand{\basedon}[1]{\begin{flushleft} {\small This chapter is based on #1.}\end{flushleft}}
\newcommand{\onbased}[1]{\begin{flushleft} {\small  #1 is based on this chapter.}\end{flushleft}}
\newcommand{\ds}{\displaystyle}
%\newcommand{\note}[1]{\textsc{#1} $\clubsuit$}
\newcommand{\co}{\textrm{co}}
%%%%%%%%%%%%%% Greek Letters %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eg}{\epsilon}
\newcommand{\zg}{\theta}
\newcommand{\ag}{\alpha}
\newcommand{\bg}{\beta}
\newcommand{\dg}{\delta}
\newcommand{\mc}{\mathcal}

\usepackage{amsfonts}
\def\Real{\mathbb{R}}
\def\Complex{\mathbb{C}}
\def\Natural{\mathbb{N}}
\def\id{\mathbb{I}}

\def\01{\{0,1\}}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\eps}{\varepsilon}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\outp}[2]{|#1\rangle\langle#2|}
\newcommand{\proj}[1]{|#1\rangle\langle#1|}
\newcommand{\ketbra}[2]{|#1\rangle\langle#2|}

\newcommand{\inp}[2]{\langle{#1}|{#2}\rangle} % inproduct, < | >
\newcommand{\braket}[2]{\langle #1|#2\rangle}

\newcommand{\rank}{\operatorname{rank}}

\newtheorem{conjecture}{Conjecture}
\newtheorem{fact}{Fact}

\newtheorem{lemmaApp}{Lemma A.}
\newtheorem{corollaryApp}{Corollary A.}

\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mB}{\mathcal{B}}


\newenvironment{sdp}[2]{
\smallskip
\begin{center}
\begin{tabular}{ll}
#1 & #2\\
subject to
}
{
\end{tabular}
\end{center}
\smallskip
}

\newcommand{\ens}{\mathcal{E}}
\newcommand{\Y}{|\mY|}
\newcommand{\psucRAC}{P^{\rm uncert}}
\newcommand{\psuc}{P^{\rm succ}}
\newcommand{\pgame}{{P^{\rm game}}}
\newcommand{\pgameMAX}{{P^{\rm game}_{\rm max}}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\sx}{\mathcal{S}_x}
\newcommand{\hmin}{\ensuremath{H}_{\infty}}

\newcommand{\stateSet}{\mathscr{S}}


\newcommand{\secchsh}{\ref{sec:chsh}}
\newcommand{\nn}[1]{\textcolor{magenta}{nelly: #1}}
\newcommand{\mcomment}[1]{{\sf [#1]}\marginpar[\hfill !!!]{!!!}}
\newcommand{\steph}[1]{{\textcolor{blue}{steph: #1}}}
\newcommand{\jono}[1]{\textcolor{blue}{jono: #1}}
\newcommand{\mh}[1]{\textcolor{red}{mh: #1}}
\newcommand{\pc}[1]{\textcolor{green}{\tt Piotr: #1}}
\newcommand{\fer}[1]{\textcolor{brown}{\tt Fernando: #1}}
\newcommand{\xstr}{{\vec{x}_{s,a}}}
\newcommand{\str}{{\vec{x}}}
\newcommand{\vstr}{x}
\newcommand{\vxstr}{{x_{s,a}}}
\newcommand{\xstrsub}{s,a}
\newcommand{\probun}[1]{P^{\rm un}(#1)}
\newcommand{\probsteer}[1]{P^{\rm st}(#1)}

\newcommand{\prob}[1]{p(#1)}

\newcommand{\good}{\mathcal{G}}
\newcommand{\bstate}[1]{\sigma_{\xstrsub}^{#1}}
\newcommand{\xor}{XOR}
%\newcommand{\eeq}{\end{align}}
%\newcommand{\beq}{\begin{align}}
\newcommand{\avgb}{\rho}
\newcommand{\icaus}{I_{caus}}
\newcommand{\irac}{I_{rac}}
\newcommand{\unop}{Q}
\newcommand{\supl}{Appendix}
%\newcommand{\supl}{Supplementary Materials}
\newcommand{\stateset}{\mathcal{F}_{s}}
\newcommand{\badproj}{\Pi_{bad}}

\newcommand{\setA}{\mathcal{A}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\secxor}{I}

\newcommand{\dist}[2]{{\cal D}(#1\rangle#2)}

\def\<{\langle}
\def\>{\rangle}
\def\ot{\otimes}
\def\ermax{E_R^{\max}}
\def\esmax{E_S^{\max}}
\def\ecal{{\cal E}}
\def\hcal{{\cal H}}
\def\ecalr{{\ecal_R}}
\def\etaE{\eta_{E-E_S}}
\def\rhor{\rho_R}
\def\rhos{\rho_S}
\def\gibbs{\tau_\beta}
\def\final{\rho'}
\def\ergotropymin{F_\epsilon^{min}}
\def\ergotropymax{F_\epsilon^{max}}
\def\gmin{G_\epsilon^{min}}
\def\gmax{G_\epsilon^{max}}
\def\supthermomaj{C}
\def\supdistillation{D}
\def\supformation{D}
\def\supparadigm{A}
\def\supprocesses{E}

\def\rhodec{\omega}
\def\s{\,\,\,\,}
\def\dmin{D_{min}}
\def\dmax{D_{max}}
\def\dmine{D^\epsilon_{min}}
\def\dmaxe{D^{\epsilon}_{max}}
\def\wit{\psi_W}
\def\witi{0}
\def\initial{\rho}
\def\Hw{\hat{W}}
\def\Hin{H}
\def\Hout{H'}
\def\Zout{Z'}
\def\mainsection{Main Section}
\newcommand{\alfree}[1]{F_\alpha(#1,\gibbs)}
\newcommand{\qalfree}{{\hat F}}
%_\alpha(#1,H)}
% oh no, I can't believe we're hatting, especially here!
\newcommand{\qalfreesimple}{{\tilde F}}
%_\alpha(#1,H)}
%Michal's defs
\def\fmin{F_{\rm min}}
\def\fmax{F_{\rm max}}
\def\tauout{\tau'}
\def\ep{\epsilon}
\newcommand{\sgn}{\operatorname{sgn}}
\def\qrenyi{S}
\def\qrenyisimple{\tilde S}
% jono'ss
\def\trumpd{\rm D_{work}}
\def\catalyst{\sigma}
\def\expbound{\exp(-\Omega(\sqrt{\log(N)}))} 

\def\gibbsin{\rho_\beta^{(0)}}
\def\gibbsout{\rho_\beta^{(1)}}

\def\genFs{generalized free energies}




%\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1} (restatement)}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother






\newreptheorem{thm}{Theorem}
\newreptheorem{lem}{Lemma}



